Code Documentation and Analysis to Secure Software Development

We present the Code Documentation and Analysis Tool (CoDAT). CoDAT is a tool designed to maintain consistency between the various levels of code documentation, e.g. if a line in a code sketch is changed, the comment that documents the corresponding code is also changed. That is, comments are linked and updated so as to remain internally consistent and also consistent with the code. By flagging "out of date" comments, CoDAT alerts the developer to maintain up-to-date documentation. We use a large language model to check the semantic consistency between a fragment of code and the comments that describe it. Thus we also flag semantic inconsistency as well as out of date comments. This helps programers write code that correctly implements a code sketch, and so provides machine support for a step-wise refinement approach, starting with a code sketch and proceeding down to code through one or more refinement iterations. CoDAT is implemented in the Intellij IDEA IDE where we use the Code Insight daemon package alongside a custom regular expression algorithm to mark tagged comments whose corresponding code blocks have changed. CoDAT's backend is structurally decentralized to allow a distributed ledger framework for code consistency and architectural compilation tracking.

==> appendices.tex <==

\clearpage

\appendix

%Appendices
% 1. Userguide for CoDAT 
% 2. Link to Example Code
% 3. Link to Project Code
% 4. AI program output 

%\section{User manual for CoDAT}
\input{manual}


\section{Example Project Code}

% Project code used as an example 

\section{Appendix Plugin Code}

% Source code for plugin here along with link for full implementation (Boilerplate, etc.)




==> methodology.tex <==

\section{Methodology}

% Discuss how to integrate source control with dynamic code comment management`

Our focus with CoDAT is to explore the junction between code documentation and stateful change tracking. Oftentimes developers may change the functionality of a program without updating the inline comments or code sketches. While wikis may serve as a substitute for some developers, we believe that inline code commenting is an essential practice in any code base, especially large projects. 

% Guarantees code coverage by covering the entire program unless it's seperated by tags

% Compare current version with the file versioning system.
% Create a slide deck (Using with cyber security, company liability, etc...)

\begin{figure}[!htp]
\centering
\includegraphics[width=\linewidth]{img/CodeReview_CoDAT.png}
\caption{Code Reviews with CoDAT}
\label{fig1}
\end{figure}

As shown in Figure \ref{fig1}, CoDAT provides developers with the ability to be notified in real-time when inline code comments or sketches needs updating. While CoDAT does not block the user from not updating the inline comment or sketch, CoDAT will persistently alert the user that a code change occurred for a related code sketch or comment.





==> related.tex <==

\section{Related Works}

\subsection{Fuzzing}
In 2022, Beaman et al.\cite{BEAMAN2022102813} Published a survey on the state and direction of software fuzzing. This paper highlights the importance of code coverage and the flexibility needed to adapt to a multitude of fuzzing scenarios. The paper also mentions the importance of distributed settings in cases where resource limitations exist. Interestingly, the solution the authors present is to use a white-box approach rather than a black-box in terms of testing\cite{10.1145/2970276.2970316}. 

Code coverage implementations currently focus on multi-processor, single architecture models. Mammo et al. \cite{6519726} published a paper in 2012 describing a novel approach to a multi-processor based code coverage tool. This approach simulates program traces throughout a multi-processor architecture. 

% Be careful with opening quotes, be sure to replace it with two single quotes to show properly
Parallel fuzz testing systems is another solution to solve the resource limitation problem\cite{9939114}. As a, ''de-facto standard for fuzzing''\cite{10.1145/3580596}, American Fuzzy Lop, or AFL, uses a per core-based approach to parallelization\cite{AFL}. In other words, each instance of AFL uses one CPU core, so parallelization can occur on a multi-core system.

Parallelism optimizations have primarily been centered around improving the program flow and state selection. In particular, Xu et al. \cite{10.1145/3133956.3134046} published a paper where in-part they optimized AFL using a novel system call, shared memory logs, and a daemon. The underlying parallelization was not affected, simply improved using additional programming techniques. On the other hand, Ye et al. \cite{8668503} proposed a prioritization algorithm that changed the order in which the program is fuzzed. However, the underlying parallelism of AFL remains intact. 

In addition to the aforementioned optimizations, Li et al. \cite{10.1145/3239576.3239615} published a paper in 2018 suggesting two improvements to the way parallelism and distribution occurs within AFL. First, the author suggests reducing the size of data used to maintain synchronization. The second is to introduce static analysis prior to the fuzz test. 

The existing format of parallelism as defined in AFL is well established. The focus of this paper is to integrate the existing technique of parallelism with the DLT. However, when integrating parallelism with DLT, proof-of-work (PoW) or equivalent algorithms is needed to enforce authenticity and prevent cheating. 

Cheat proofing traditionally has been defined as discrete methods to mathematically prove authenticity via PoW algorithms \cite{golle2001uncheatable} \cite{1281562}. However, given the arbitrary nature of fuzzing, a more robust approach is needed to verify work. Jang et al. \cite{10.1145/3545948.3545971} proposed a solution through the use of Proof-of-Fuzzing-Work (PoFW). With PoW mechanisms typically restricted to cryptocurrency applications, PoFW implements PoW in arbitrary computation.

\subsection{Smart Contract Fuzzing}
When applied to smart contracts, fuzzing helps detect flaws in the contract code that could lead to security breaches or unintended behavior. By subjecting the smart contract to various inputs and edge cases, fuzzing can reveal unforeseen scenarios that may not have been thoroughly tested during traditional development processes. This proactive approach can significantly reduce the risk of critical security vulnerabilities and improve the overall reliability of smart contracts deployed on the blockchain. By continuously fuzzing smart contracts and addressing the identified issues, developers can ensure that their applications are better prepared to handle real-world scenarios and adversarial attacks, ultimately bolstering the confidence of users and stakeholders in the blockchain ecosystem.

Therefore, within the Blockchain, current fuzzing applications primarily focus around testing smart contracts for vulnerabilities \cite{10.1145/3238147.3238177}\cite{choi2021smartian}\cite{grieco2020echidna}\cite{liao2019soliaudit}\cite{nguyen2020sfuzz}\cite{wustholz2020harvey}. Smart contracts are essential in enforcing and monitoring activity within a decentralized network. As a result, they are a prime target for attack and thus serve as a important surface for fuzz testing. 

Smart contract fuzzing is a technique used to identify vulnerabilities and potential bugs in smart contracts by subjecting them to a large number of random inputs and scenarios. It is a form of automated testing where the smart contract is bombarded with various inputs, transactions, and function calls in an attempt to find unexpected behaviors or security flaws.

The process of smart contract fuzzing involves generating a wide range of test cases, often using tools or scripts that create random or mutated inputs. These inputs are then fed into the smart contract, and its behavior is observed. The goal is to identify edge cases, boundary conditions, and other scenarios that may not have considered during the manual testing phase.

For example, by fuzzing smart contracts vulnerabilities such as integer overflow/underflow, reentrancy issues, unexpected behavior due to overflow/underflow can be discovered. Therefore, fuzzing is an essential part of the security assessment process for smart contracts because it simulates real-world conditions and allows for the identification of potential weaknesses that may not be apparent during traditional manual code reviews.

\subsection{Automatic Comment Generation}

% CloCom: Mining Existing Source Code for Automatic Comment Generation

\cite{7081848}

\subsection{Comment Reuse Parsing}

% Automatic Generation of Code Comments Based on Comment Reuse and Program Parsing

\cite{9095968}

